Constraint Programming Approaches to the Discretizable Molecular Distance Geometry Problem

The Distance Geometry Problem (DGP) seeks to find positions for a set of points in geometric space when some distances between pairs of these points are known. The so-called discretization assumptions allow to discretize the search space of DGP instances. In this paper, we study the Discretizable Molecular Distance Geometry Problem whose feasible solutions provide a discretization scheme for the DGP. We propose the first constraint programming formulations as well as a set of checks for proving infeasibility, domain reduction techniques, symmetry breaking constraints and valid inequalities. Our computational results indicate that our formulations outperform the state-of-the-art integer programming formulations, both for feasible and infeasible instances.

==> CDrelax.tex <==
\begin{landscape}
\renewcommand\arraystretch{0.8}
\begin{center}
	\small
	\begin{longtable}{cccl rr rr rr rr}
					\caption{Results for $\IPCD$ and $\Unorderedrelax$ on small instances.}
		\label{table:CDrelax} \\
		\toprule
 &  &  &  &\multicolumn{2}{c}{ $\Unorderedrelax$} & \multicolumn{2}{c}{\# Cliques} &  \multicolumn{2}{c}{Time} &  \multicolumn{2}{c} {BB Nodes} \\
	 \cmidrule(lr){5-6}
 \cmidrule(lr){7-8}
 \cmidrule(lr){9-10}
  \cmidrule(lr){11-12}
% \cmidrule(lr){12-14}
% \cmidrule(lr){15-17}
$n$ & $\density$ & Inst. & Status & Solved & DMDGP found & $\IPCD$ & $\Unorderedrelax $ &  $\IPCD$ & $\Unorderedrelax$ &  $\IPCD$ & $\Unorderedrelax$ \\
\midrule
20 & 0.3 & 1 & Infeas. & - & - & 168 & 7 & \textBF{0.00} & 0.00 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 48 & 2 & \textBF{0.00} & 0.00 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 96 & 4 & \textBF{0.00} & 0.00 & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Infeas. & - & - & 1656 & 69 & 4.13 & \textBF{2.08} & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 1920 & 80 & 5.66 & \textBF{1.83} & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 1272 & 53 & 1.86 & \textBF{0.00} & 0 & 0 \\*[0.18cm]
 & 0.7 & 1 & Feas. & Yes & No & 13872 & 578 & TL & \textBF{5308.77} & 0 & 6287 \\
 &  & 2 & Feas. & Yes & No & 12000 & 500 & TL & \textBF{2217.26} & 0 & 7172 \\
 &  & 3 & Feas. & Yes & No & 13872 & 578 & TL & \textBF{2105.65} & 0 & 3579 \\
 \midrule
25 & 0.3 & 1 & Infeas. & - & - & 288 & 12 & \textBF{0.00} & 0.00 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 216 & 9 & \textBF{0.00} & 0.00 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 96 & 4 & \textBF{0.00} & 0.00 & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Infeas. & - & - & 4776 & 199 & 0.03 & \textBF{0.01} & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 4368 & 182 & \textBF{962.72} & 4095.70 & 0 & 7968 \\
 &  & 3 & Infeas. & - & - & 3960 & 165 & \textBF{632.05} & TL & 0 & 18996 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 36360 & 1515 & MEM & TL & - & 287 \\
 &  & 2 & Feas. & No & - & 34344 & 1431 & MEM & TL & - & 180 \\
 &  & 3 & Feas. & Yes & No & 32856 & 1369 & MEM & \textBF{4536.87} & - & 333 \\
 \midrule
30 & 0.3 & 1 & Infeas. & - & - & 264 & 11 & \textBF{0.00} & 0.01 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 240 & 10 & \textBF{0.00} & 0.01 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 360 & 15 & \textBF{0.00} & 0.01 & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 10896 & 454 & TL & TL & 0 & 3742 \\
 &  & 2 & \textbf{Unsol.} & - & - & 9264 & 386 & TL & TL & 0 & 3293 \\
 &  & 3 & Feas. & - & - & 9960 & 415 & TL & TL & 0 & 2866 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 73872 & 3078 & MEM & TL & - & 12 \\
 &  & 2 & Feas. & No & - & 72888 & 3037 & MEM & TL & - & 6 \\
 &  & 3 & Feas. & No & - & 76488 & 3187 & MEM & TL & - & 3 \\
 \midrule
35 & 0.3 & 1 & Infeas. & - & - & 864 & 36 & \textBF{0.00} & 0.01 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 576 & 24 & \textBF{0.00} & 0.01 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 696 & 29 & \textBF{0.00} & 0.01 & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 18888 & 787 & TL & TL & 0 & 1457 \\
 &  & 2 & Feas. & No & - & 21408 & 892 & TL & TL & 0 & 1828 \\
 &  & 3 & Feas. & No & - & 20304 & 846 & TL & TL & 0 & 605 \\
 & 0.7 & 1 & Feas. & No & - & 143616 & 5984 & MEM & TL & - & 0 \\*[0.18cm]
 &  & 2 & Feas. & No & - & 151056 & 6294 & MEM & TL & - & 0 \\
 &  & 3 & Feas. &  &  & 140976 & 5874 & MEM & TL & - & 0 \\
 \midrule
40 & 0.3 & 1 & Infeas. & - & - & 1776 & 74 & \textBF{0.00} & 0.01 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 816 & 34 & \textBF{0.00} & 0.01 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 1344 & 56 & \textBF{0.00} & 0.01 & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 34680 & 1445 & MEM & TL & - & 56 \\
 &  & 2 & Feas. & No & - & 37056 & 1544 & MEM & TL & - & 72 \\
 &  & 3 & Feas. & No & - & 35160 & 1465 & MEM & TL & - & 48 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 250608 & 10442 & MEM & TL & - & 0 \\
 &  & 2 & Feas. & No & - & 265440 & 11060 & MEM & TL & - & 0 \\
 &  & 3 & Feas. & No & - & 256224 & 10676 & MEM & TL & - & 0 \\
 \midrule
45 & 0.3 & 1 & Infeas. & - & - & 2136 & 89 & \textBF{0.01} & 0.02 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 2472 & 103 & \textBF{0.01} & 0.02 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 2376 & 99 & 1.89 & \textBF{0.02} & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 55032 & 2293 & MEM & TL & - & 0 \\
 &  & 2 & Feas. & No & - & 56664 & 2361 & MEM & TL & - & 2 \\
 &  & 3 & Feas. & No & - & 54360 & 2265 & MEM & TL & - & 5 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 412416 & 17184 & MEM & MEM & - & - \\
 &  & 2 & Feas. & No & - & 404088 & 16837 & MEM & MEM & - & - \\
 &  & 3 & Feas. & No & - & 423720 & 17655 & MEM & MEM & - & - \\
 \midrule
50 & 0.3 & 1 & Infeas. & - & - & 4536 & 189 & 0.02 & \textBF{0.02} & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 3768 & 157 & 7.04 & \textBF{0.42} & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 4296 & 179 & \textBF{0.02} & 0.03 & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 87552 & 3648 & MEM & TL & - & 0 \\
 &  & 2 & Feas. & No & - & 83544 & 3481 & MEM & TL & - & 0 \\
 &  & 3 & Feas. & No & - & 82680 & 3445 & MEM & TL & - & 0 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 621552 & 25898 & MEM & MEM & - & - \\
 &  & 2 & Feas. & No & - & 657264 & 27386 & MEM & MEM & - & - \\
 &  & 3 & Feas. & No & - & 662352 & 27598 & MEM & MEM & - & - \\
 \midrule
55 & 0.3 & 1 & Infeas. & - & - & 5328 & 222 & \textBF{14.13} & 539.85 & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 4896 & 204 & \textBF{0.03} & 0.04 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 5568 & 232 & 0.03 & \textBF{0.03} & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 127608 & 5317 & MEM & TL & - & 0 \\
 &  & 2 & Feas. & No & - & 129600 & 5400 & MEM & TL & - & 0 \\
 &  & 3 & Feas. & No & - & 126168 & 5257 & MEM & TL & - & 0 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 958200 & 39925 & MEM & MEM & - & - \\
 &  & 2 & Feas. & No & - & 946944 & 39456 & MEM & MEM & - & - \\
 &  & 3 & Feas. & No & - & 994824 & 41451 & MEM & MEM & - & - \\
 \midrule
60 & 0.3 & 1 & Infeas. & - & - & 8976 & 374 & \textBF{4061.37} & TL & 0 & 0 \\
 &  & 2 & Infeas. & - & - & 6888 & 287 & \textBF{26.81} & 371.402 & 0 & 0 \\
 &  & 3 & Infeas. & - & - & 8424 & 351 & 0.07 & \textBF{0.05} & 0 & 0 \\*[0.18cm]
 & 0.5 & 1 & Feas. & No & - & 188496 & 7854 & MEM & TL & - & 0 \\
 &  & 2 & Feas. & No & - & 171840 & 7160 & MEM & TL & - & 0 \\
 &  & 3 & Feas. & No & - & 184728 & 7697 & MEM & TL & - & 0 \\*[0.18cm]
 & 0.7 & 1 & Feas. & No & - & 1406256 & 58594 & MEM & MEM & - & - \\
 &  & 2 & Feas. & No & - & 1363296 & 56804 & MEM & MEM & - & - \\
 &  & 3 & Feas. & No & - & 1379184 & 57466 & MEM & MEM & - & - \\
\bottomrule
\end{longtable}
\end{center}
\end{landscape}

